Snowmass Cosmic Frontiers 6 (CF6) Working Group Summary --The Bright Side of the Cosmic Frontier: Cosmic Probes of Fundamental Physics

Report of the CF6 Working Group at Snowmass 2013. Topics addressed include ultra-high energy cosmic rays, neutrinos, gamma rays, baryogenesis, and experiments probing the fundamental nature of spacetime.

==> CF6/CF6_Intro.tex <==
\title{The Bright Side of the Cosmic Frontier: Cosmic Probes of Fundamental Physics (CF6).}
\maketitle
\section{Executive Summary (1-2 pages)}

The Bright Side of the Cosmic Frontier (CF6) addresses fundamental questions related to the nature of high-energy interactions and the structure of space and time through cosmic probes other than dark matter and dark energy. Cosmic Probes include 

$\bullet$ Standard Model particles (Cosmic Rays, Gamma Rays, and Neutrinos) that can reach energies much greater than those accessible in artificial accelerators; 

$\bullet$ the mechanisms behind cosmic accelerators and the limits of their extreme energy reach; 

$\bullet$ searches for new particles that may reach the Earth or produce indirect signatures; 

$\bullet$ the origin of the matter-antimatter asymmetry; and

$\bullet$ tests of space and time properties (extra-dimensions, Lorenz invariance violations, and holography).


The field has ample room for ground-breaking discoveries. Some recent results include the detection by the Fermi and AGILE space missions of the smoking gun of cosmic ray acceleration through the $\pi^0 \to \gamma \gamma $  signal in supernova remnants W44 and IC44 \cite{FermiW44}; the first detection of  neutrinos from 50 TeV to 1 PeV by Icecube \cite{BertErnie}; and the precise positron fraction measurement of the Alpha Magnetic Spectrometer \cite{AMSpositrons}. 

$\bullet$ Increased sensitivity over a wide range of energies will be key in understanding the limits of cosmic accelerators and their ability to probe physics beyond the SM. 

$\bullet$ R\&D needs in the field include more sensitive photodetectors; [[ADD NEEDS HEREÉ]]. 

$\bullet$ The field is driven by international collaborations of particle physicists who utilize similar techniques and technologies to those used by other HEP experiments. 

$\bullet$ Theoretical work in this field is very important to distinguishing astrophysical effects from new fundamental physics, and to make connections between new particle physics ideas and what can be probed with cosmic particles.

$\bullet$ Energy and Intensity frontier probes of CO violation may help illuminate the question of the origin of the matter-antimatter asymmetry in the Universe.

$\bullet$ Energy Frontier probes of hadronic interactions in the forward direction can narrow extrapolation gaps to 100 TeV CM scales reached by extremely energetic cosmic rays

$\bullet$ Intensity Frontier probes of the neutrino sector are strongly related to the nascent cosmic neutrino observations at PeV scales.

$\bullet$ A confirmed positive result on that extend the limits of the known space and time properties will be a revolutionary discovery (e.g., extra-dimensions, Lorenz invariance violations, and holography).

[[Figure 1a shows the current reach of CF6-A experiments.]]

[[Figure 1b shows the future opportunities in CF6-A.]]

\subsection{Elevator answer to Tough Questions}

\noindent {\bf What will it take to answer the following CF6 generated questions:}

\noindent {\it What is the origin of cosmic rays?}

{\it The origin of Galactic Cosmic Rays}

Answer

{\it The origin Extragalactic Ultrahigh to Extreme Energy Cosmic Rays?}

Answer

{\it  How do cosmic accelerators work?}

Answer

\noindent {\it What are the sources of very high energy neutrinos?}

Answer

\noindent {\it What can cosmic rays, neutrinos, and photons tell us about particle physics beyond LHC energies? }

Answer

\noindent {\it What can we learn from the extragalactic background light?}

Answer

\noindent {\it What is the origin of the matter-antimatter asymmetry?}

Answer

\noindent {\it How can we probe the fundamental nature of spacetime?}

Answer

	{\it Is Lorentz invariance violated at extreme energies?}

Answer

\noindent {\it What can we learn about fundamental physics from astrophysical gamma-ray beams?}

Answer

\medskip

\noindent {\bf  Relevant Tough Questions to CF6 } 

\noindent {\it G1. How do we exploit science opportunities at the interfaces between the Frontiers?}

Common technics and instrumentation; Hadronic interaction models for UHECRs tests at LHC; neutrino interactions at very high energies; matter-antimatter asymmetry in the early universe and neutrino mixing; 
\medskip


\noindent {\it IF10. What do the neutrino parameters that can be measured over the coming decade (delta CP, hierarchy) tell us? Measuring the quark mixing parameters (which are sometimes overconstrained and testable for consistency) has not yet revolutionized our understanding of flavor structure and the matter-antimatter asymmetry. How might the neutrino sector be different? }

Answer

\medskip
\noindent {\it  IF13. Imagine that one measures the CP violating phase in the neutrino sector to be 85 degrees (for example). What does this imply for the hypothesis that the matter-anti-matter asymmetry is due to leptogenesis? What is the next measurement that one should make to clarify this relation? }

Answer

\medskip
\noindent {\it CF33. What expertise can HEP experimentalists deploy in telescope-based experiments? Where are the overlaps?}

Answer

\medskip
\noindent {\it CF34. What are the roles of cosmic-ray, gamma-ray, and neutrino experiments for particle physics? What future experiments are needed in these areas and why? Are there areas in which these can have a unique impact?}

Answer

\medskip
\noindent {\it CF35. What will it take to identify the mechanism for baryogenesis or leptogenesis? Are there scenarios that could conceivably be considered to be established by experimental data in the next 20 years?}

Answer

\medskip
\noindent {\it CF36. What are the leading prospects for detecting GZK neutrinos? What experimental program is required to do this in the next 5 years, 10 years, 20 years, and how important is this?}

Answer


\section{Introduction (2-3 pages)}

The Cosmic Frontier number 6, named Cosmic Probes of Fundamental Physics, was charged with summarizing current knowledge and identifying future opportunities (both experimental and theoretical) in the use of astrophysical probes of fundamental physics. Because of the breadth of this area of research CF6 has been subdivided into 3 main topical areas:

\begin{itemize}
\item	CF6-A Cosmic Rays, Gamma Rays and Neutrinos (conveners: Gus Sinnis, Tom Weiler)
\item	CF6-B The Matter of the Cosmological Asymmetry (convener: Ann Nelson)
\item	CF6-C Exploring the Basic Nature of Space and Time (conveners: Aaron Chou, Craig Hogan)
\end{itemize}

We received [[XX]] whitepapers addressing the current challenges and future opportunities in each of these fields as they relate to the other frontiers of high energy physics.

\subsection{Physics Motivation}

The Universe has a large number of cosmic accelerators that can give insight into particle interactions and fundamental physics. Understanding  the flux and energy reach of particles that reach Earth from remote places in the cosmos give an opportunity to probe physics beyond the reach of artificial laboratories. In addition to probing the limits of known interactions with cosmic probes, high sensitivity experiments can find rare long lived new particles that can change current views on the basic components of matter. 

The basic question of the matter-antimatter is another focus of this cosmic frontier. [[Ann may want to add some sentences here]]

Quantum effects of space-time are predicted to originate at the Planck scale. In standard quantum eld theory, their effects are strongly suppressed at experimentally accessible energies, so space-time is predicted to behave almost classically, for practical purposes, in particle experiments. However, new quantum effects of geometry originating at the Planck scale| from geometrical degrees of freedom not included in standard field theory| may have effects on macroscopic scales that could be measured by laser interferometers, such as the bolometer. In addition, 
cosmic particles of high energies can probe departures from Lorenz invariance and the existence of extra-dimensions on scales above the LHC.



\subsection{Summary of topical areas addressed }

\subsubsection{CF6-A Cosmic Rays, Gamma Rays and Neutrinos}

Cosmic rays, gamma rays, and neutrinos from astrophysical sources can be used to probe fundamental symmetries, particle interactions at energies not attainable on Earth, and understand the nature of particle acceleration in the cosmos. CF6-A encompasses the following topical areas:
	The Physics of Interactions Beyond Laboratory Energies (hadronic and weak interactions at high energies)
	Cosmic Particle Acceleration (origin of the cosmic radiation from GeV to ZeV, astrophysical backgrounds to fundamental physics)
	Cosmic Standard Model (SM) Particles as Probes of Fundamental Physics (violation of Lorentz invariance, extra dimensions, axions)
	New Particles (anti-nuclei, strangelets, Q-Balls, primordial black holes)
	Neutrino Physics from Astrophysics (in conjunction with the Intensity Frontier IF3: neutrino mass hierarchy, leptonic CP violation, neutrino interactions in supernovae, non-standard neutrino interactions with matter)

The relevant experiments for CF6-A are listed in TABLE 1. This field is ripe for new discoveries. Recent examples include the detection by the Fermi and AGILE space missions of a pion-zero decay produced gamma-ray signal in supernova remnants W44 and IC44 \cite{FermiW44}; the first detection of 10 TeV to PeV neutrinos by Icecube \cite{BertErnie}; and the precise positron fraction measurement of the Alpha Magnetic Spectrometer \cite{AMSpositrons}. The 


\subsubsection{CF6-B The Matter of the Cosmological Asymmetry}

The cosmological asymmetry between baryons and anti-baryons is one of the strongest pieces of evidence for physics beyond the standard model. There are diverse theoretical proposals for new physics at a range of energy scales, most of which include new sources of CP violation, and either additional baryon or lepton number violation. There are plausible theories with implications for experiments at all three frontiers. Leptogenesis theories predict new CP violation in the neutrino sector. Grand Unified theories predict proton decay. Electroweak baryogenesis models predict a cosmological phase transition which leaves traces in gravitational wave and CMB experiments, and new collider physics at or below a TeV.

Survey what we may expect to learn about the origin of matter from searches at ongoing, planned and proposed facilities such as the LHC, ILC, CLIC, muon collider, B-factories, neutrino experiments, gravitational wave experiments and CMB experiments.

\subsubsection{CF6-C Exploring the Basic Nature of Space and Time}

Space and time may be quantized at the Planck scale. Effects from this extremely high-energy realm may be studied through gravitational waves from the early universe and holographic noise.

Survey what we may expect to learn about the GUT and Planck energy scale with gravitational waves and holographic noise. Survey the theory and ongoing, planned, and proposed gravitational wave and holographic noise experiments. Examples of relevant experiments include the Holometer, LIGO, LISA, and CMB probes of early universe gravitational wave (covered in Dark Energy and CMB.)


\subsection{Upcoming Opportunities (Next Generation Facilities) }

\subsubsection{(short list that addresses questions and physics issues)}

\subsection{Answers to Tough Questions}
\pagebreak



==> CF6/executive-summary-v4short.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{center}\begin{boldmath}

%\input authorlistCF.tex
%Conveners are also listed separately in authorlist.tex

%\end{boldmath}\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newpage

\section{Cosmic Particles and Fundamental Physics} 


Over the past decade we have witnessed a revolution in our
understanding of the high-energy universe.  Some of the key
discoveries have been:
\begin{itemize}
\item Supernovae have been shown to be a source of Galactic cosmic
  rays \cite{ackermann2013a,Giuliani:2011nx,acciarri2011}.
\item Very high energy neutrinos that are likely to be astrophysical
  in origin have been observed \cite{Aartsen:2013bka}.
\item The GZK suppression \cite{Greisen:1966jv,Zatsepin:1966jv} in the cosmic-ray flux above $10^{19.5}$ eV
  has been observed \cite{Abbasi:2007sv,Abraham:2008ru,AbuZayyad:2012ru,Abraham:2010mj}.
\item The positron fraction of the cosmic rays has been measured up to
  300 GeV and provides solid evidence for a high-energy primary source
  of positrons in the Galaxy, either from dark matter annihilation or
  astrophysical processes \cite{adriani2009,acciarri2011,Aguilar:2013qda,yuksel2009}.
\item Many sites of astrophysical particle acceleration have been
  directly observed, from supermassive black holes and merging neutron
  stars, to rapidly spinning neutron stars and supernova remnants in
  our Galaxy \cite{Aharonian:2008zza,funk2012,rieger2013,tevcat}.
\end{itemize}

These discoveries have been driven by the current generation of
experiments: the IceCube neutrino detector at the South Pole \cite{Collaboration:2011ym,Halzen:2010yj}, the
Fermi gamma-ray observatory \cite{Atwood2009} and the PAMELA \cite{menn2013} and AMS experiments \cite{kounine2012}
orbiting the earth, the High Resolution FlyÕs Eye \cite{boyer2002} and Pierre Auger \cite{Abraham:2010mj}
ultra-high-energy cosmic ray experiments, and the H.E.S.S. \cite{aharonian2005}, VERITAS \cite{weekes2002},
MAGIC \cite{aleksic2011} and Milagro \cite{atkins2003} experiments in very high energy gamma rays.  Looking
forward, a new generation of instruments with greater sensitivity and
higher resolution hold the promise of making large advances in our
understanding of astrophysical processes and the fundamental physics
studied with astrophysical accelerators.  The goals for the coming
decade are:
\begin{itemize}
\item Determine the origin of the highest energy particles in the
  universe and understand the acceleration processes at work
  throughout the Universe.
\item Measure particle cross sections at energies unattainable in
  Earth-bound accelerators.
\item Measure the highest energy neutrinos that arise from
  interactions of the ultra-high-energy cosmic rays with the microwave
  background radiation.
\item Measure the extragalactic background light between 1 and 100
  microns to understand the star formation history of the Universe.
\item Measure the mass hierarchy of the neutrinos.
\item Search for physics beyond the standard model encoded in cosmic
  messengers as they cross the Universe.
\item Understand the origins of the matter antimatter asymmetry of the
  Universe.
\item Probe the fundamental nature of spacetime.
\end{itemize}

In many of these areas future progress will depend upon either the
detailed understanding of particle acceleration in the universe or the
development of methods for controlling systematic errors introduced by
our lack of understanding of these processes.  High-resolution gamma
ray measurements (spectral, angular, and temporal) of many objects and
classes of objects are needed to find the source invariant physics
that is the signal for physics beyond the standard model.  Such
measurements in conjunction with measurements at other wavelengths and
with measurements of cosmic rays, neutrinos, and gravity waves will
enable us to understand NatureÕs particle accelerators.

\underline{\bf Recommendations:}
\begin{itemize}
\item Significant U.S. participation in the CTA project \cite{cta2011}.
  U.S. scientists developed the imaging atmospheric Cherenkov
  technique.  Continued leadership in this area is possible with the
  development of novel telescope designs.  A U.S. proposal to double
  the number of mid-scale telescopes will improve the performance of
  CTA by a factor of 2-3 significantly improving the prospects for the
  indirect detection of dark matter, understanding particle
  acceleration processes, and searching for other signatures of
  physics beyond the standard model.
\item Simultaneous operation of Fermi, HAWC, and VERITAS.
  Understanding particle acceleration and separating astrophysical
  processes from physics beyond the standard model requires
  observations over a broad energy range.  The above three instruments
  will provide simultaneous coverage from 30 MeV to 100 TeV.  HAWC and
  VERITAS will simultaneously view the same sky enabling prompt follow
  up observations of transient phenomena.
\item Construction of the PINGU neutrino detector \cite{aartsen2013} at the South Pole.
  U.S. scientists have been leaders in the field of high-energy
  neutrino observations.  PINGU, by densely instrumenting a portion of
  the IceCube Deep Core array, will lower the energy threshold for
  neutrinos to a few GeV.  This will allow for a measurement of the
  neutrino mass hierarchy using atmospheric neutrinos.
\item Continued operation of the Auger and TA air shower arrays with
  upgrades to enhance the determination of the composition and
  interactions of cosmic rays near the energy of the GZK suppression,
  and flight of the JEM-EUSO mission \cite{Adams:2013vea,TheJEM-EUSO:2013vea} to extend observations of the
  cosmic ray spectrum and anisotropy well beyond the GZK region.
\item Construction of a next-generation ultra-high energy GZK neutrino
  detector either to detect GZK neutrinos \cite{berezinsky2006} and constrain the
  neutrino-nucleon cross section at these energies \cite{Klein2013,hooper2002,Borriello2008,Connolly2011,Romero2009}, or rule out all
  but the most unfavorable parts of the allowed parameter space.
\end{itemize}

\subsection{Ultra-High-Energy Cosmic Rays}

HiRes  \cite{Abbasi:2007sv}, Auger  \cite{Abraham:2008ru,Abraham:2010mj}, and the Telescope Array (TA) \cite{AbuZayyad:2012ru} have established the
existence of a suppression of the spectrum at the highest energies
(above $\sim6\times 10^{19}$ eV ) as predicted by Greisen, Zatsepin,
and Kuzmin (GZK) in 1966 \cite{Greisen:1966jv,Zatsepin:1966jv}.  The GZK suppression is an example of the
profound links between different regimes of physics, connecting the
behavior of the highest-energy particles in the Universe to the cosmic
microwave background radiation, and can be explained by the sub-GeV
scale physics of photo-pion production occurring in the extremely
boosted relativistic frame of the cosmic ray.  A similar phenomenon
occurs for primary nuclei due to excitation of the giant dipole
resonance, resulting in photo-disintegration.  For iron nuclei, this
occurs at about the same energy per particle as the photo-pion process
does for protons.

The composition of cosmic rays and their interactions with air nuclei
may be probed by studies of the depth of shower maximum, $X_{max}$ \cite{ellsworth1982, baltrusaitis1984,Collaboration:2012wt}.
The mean value of $X_{max}$ rises linearly as a function of the log of
the energy, and depends on the nature of the primary particle, the
depth of its first interaction, and the multiplicity and inelasticity
of the interactions as the shower evolves.  Lower energy observations
of $X_{max}$ indicate that the composition becomes lighter as the
energy increases toward $\sim10^{18.3}$ eV \cite{FlysEye93,gaisser1993,bird1994}, which suggests that
extragalactic cosmic rays are mainly protons.  However, at higher
energies the Auger ObservatoryÕs high quality, high-statistics sample
exhibits the opposite trend, along with a decreasing spread in
$X_{max}$ with increasing energy \cite{Abraham:2010mj,Abreu:2013env}.  Using current simulations and
hadronic models tuned with LHC forward data, this implies the
composition is becoming gradually heavier above $10^{18.5}$ eV.  A
trend toward heavier composition could reflect the apparent GZK
suppression being in fact the endpoint of cosmic acceleration in which
there is a maximum magnetic rigidity for acceleration, resulting in
heavy nuclei having the highest energy per particle.

Cosmic rays can be used to probe particle physics at energies far
exceeding those available at the LHC.  An alternative explanation for
the observed behavior of $X_{max}$ is a change in particle
interactions not captured in event generators tuned to LHC data.
Auger measurements using three independent methods find that these
models do not describe observed showers well.  For example, the
observed muon content of showers measured in hybrid events at Auger is
a factor 1.3 to 1.6 higher larger than predicted \cite{AugerMuonICRC13}.  TA also observes a
calorimetric energy that is about 1.3 times higher than that inferred
from their surface detector using these models.  An example of a novel
phenomenon that may explain these observations is the restoration of
chiral symmetry in QCD  \cite{Farrar:2013sfa}.

A critical step in fully understanding the $X_{max}$ observations is
to identify and correct the deficiencies in the beyond-LHC physics
used in modeling showers.  This requires continued operation of
current hybrid detectors such as Auger and TA with upgrades to enable
improved multiparameter studies of composition and interactions on a
shower-by-shower basis.  Enhancements of the surface detectors are
particularly valuable because of the tenfold higher duty cycle than
for fluorescence or hybrid operation.

Observations from space can extend studies of the spectrum and
anisotropy beyond the GZK region with high statistics.  Current
ground-based observatories have observed hints of correlation of
cosmic ray arrival directions with the local distribution of matter \cite{Cronin:2007zz,Abraham:2007si,Abreu:2010ab,AugerICRC-HL12,AbuZayyad:2012hv,TinyakovTAanisoICRC13}, but higher statistics trans-GZK observations are required to identify
sources. In addition, the question of whether the spectrum flattens
again above the GZK suppression or continues to fall will distinguish
between the GZK and acceleration limit scenarios.  The JEM-EUSO
mission has an instantaneous collecting area of $\sim$40  \cite{Adams:2013vea,TheJEM-EUSO:2013vea} times that of
existing ground-based detectors and, taking duty cycle into account,
will increase the collecting area above the GZK suppression energy by
nearly an order of magnitude.

\subsection{Neutrinos}

IceCube has recently reported the detection
of two neutrinos with energies above 1 PeV and 26 events above 30 TeV
with characteristics that point to an astrophysical origin \cite{Aartsen:2013bka}.  These
exciting results herald the beginning of the era of high-energy
neutrino astronomy, and initiating the study of ultra-long baseline
high-energy neutrino oscillations.  Neutrino data complements
observations of cosmic rays and gamma rays due to their origin in the
decays following high-energy hadronic interactions and their weak
couplings.  Several acute issues in particle physics and astrophysics
can be addressed by neutrino experiments.

\underline{\em GZK Neutrinos} Neutrinos are produced by the weak
decays of the mesons and neutrons produced in the interaction of UHE
cosmic rays with the CMB \cite{berezinsky2006}.  The production of these neutrinos takes
place via well-known physics at high Lorentz boost, so robust
predictions of the neutrino flux can be made.  This flux depends on
the composition of the primary cosmic rays and the evolution of the
cosmic ray source density with redshift.  Unlike many searches, there
is a lower limit on the expected flux.  Current detectors such as
IceCube \cite{abbasi2011,ishihara2012}, Auger \cite{Abreu:2011zze}, RICE \cite{Kravchenko:2011im} and ANITA \cite{Hoover:2010qt,barwick2006} 
have begun to probe the highest predicted values of the neutrino flux.  Next generation experiments
such as ARA, ARIANNA, and EVA can increase our sensitivity by about
two orders of magnitude, and will either detect GZK neutrinos or rule
out much of the parameter space.  If GZK neutrinos are detected, the
event rate as a function of zenith angle can be used to measure the
neutrino-nucleon cross section and constrain models with enhanced
neutrino interactions at high energy.

\underline{\em Atmospheric Neutrinos and the Neutrino Mass Hierarchy}
PINGU \cite{aartsen2013} is a proposed high-density infill of the IceCube detector with a
reduced energy threshold of a few GeV, employing the rest of IceCube
as an active veto.  PINGU has sensitivity to atmospheric $\nu_{\mu}$
over a range of values of L/E spanned by the variation in the distance
to the production region as a function of zenith angle and the energy
spectrum of atmospheric neutrinos.  Preliminary studies of PINGU
indicate that over these values of L/E, atmospheric $\nu_{\mu}$
oscillations can be used to determine the neutrino mass hierarchy with
3-5$\sigma$ significance with two years of data with a 40 string
detector \cite{aartsen2013} .

\underline{\em Supernova Neutrinos} The Long Baseline Neutrino
Experiment \cite{Adams:2013qkq} will consist of a large (10-35 kTon) liquid argon time
projection chamber located at 4850 feet depth at the Homestake mine in
South Dakota. Collective oscillations of neutrinos as they traverse
the neutrinosphere lead to a spectral swap that leaves a signature in
the energy spectrum of electron neutrinos that is dependent upon the
neutrino mass hierarchy \cite{duan2006,duan2007,duan2010,dasgupta2009}.  In the event of a Galactic supernova,
sufficient numbers of events would be detected to both measure the
neutrino mass hierarchy and to elucidate the supernova mechanism.


\subsection{Gamma Rays}

High-energy gamma rays provide a unique view into the most extreme
environments in the universe, allowing one to probe particle
acceleration processes and the origin of the Galactic and
extragalactic cosmic rays.  Active galactic nuclei (AGN), supermassive
black holes emitting jets of highly relativistic particles along their
rotation axis, have been shown to be sites of particle acceleration \cite{Aharonian:2008zza,funk2012,rieger2013,tevcat}.
Outstanding issues in the acceleration processes include: the nature
of the accelerated particles (hadronic or leptonic), the role of shock
acceleration versus magnetic reconnection, and the formation and
collimation of astrophysical jets \cite{boettcher2007,Bykov:2012ca}.  Answers to these questions will
come from higher resolution measurements in the GeV-TeV regime,
multi-wavelength campaigns with radio, x-ray, and gamma-ray
instruments, multi-messenger observations with gamma rays, ultra-high
energy cosmic rays, neutrinos, and potentially gravitational
waves. Understanding these extreme environments and how they
accelerate particles is of fundamental interest.  In addition, these
high-energy particle beams, visible from cosmologically interesting
distances, allow us to probe fundamental physics at scales and in ways
that are not possible in earth-bound particle accelerators.

Recently, Fermi \cite{ackermann2013a} and AGILE \cite{Giuliani:2011nx} measured the energy spectra of the supernova
remnants W44 and IC44 Ð the decrease in the gamma-ray flux below the
pion mass in these sources is clear evidence for hadronic
acceleration.  This is the clearest evidence to date that some
Galactic cosmic rays are accelerated in supernova remnants.  The
detection of high-energy neutrinos from a cosmic accelerating would be
a smoking gun signature of hadronic acceleration.  In the absence of
multi-messenger signals multi-wavelength energy spectra (x-ray to TeV)
can test both leptonic models, where the high-energy emission is
derived from inverse Compton scattering of the x-ray synchrotron
emission, and hadronic models, where gamma rays result from pion
decays or proton synchrotron radiation.

\underline{\em Backgrounds to dark matter searches.} Understanding the
origin of the Galactic VHE gamma rays is critical in the
interpretation of some signatures of dark matter annihilation.  The
recent results from PAMELA \cite{adriani2009} and AMS \cite{Aguilar:2013qda} of the increasing positron fraction
with energy is a clear signal that the current model of secondary
production and transport through the Galaxy is not correct.  There are
three potential explanations for this signal: a new astrophysical
source of positrons \cite{Hooper:2008kg,Linden:2013mqa}, modified propagation of cosmic rays or secondary
production in the source \cite{Zirakashvili:2011sc,PhysRevD.82.023009}, or dark matter annihilation \cite{turner1990}.  An
astrophysical source of positrons, pulsar wind nebula (PWN), is now
known to also lead to an increasing positron fraction at high
energies.  Observations of the Geminga PWN in the TeV band by Milagro \cite{abdo2009b}
have been used to normalize the flux of positrons in our local
neighborhood from this source.  The calculated positron fraction is an
excellent match to the data \cite{yuksel2009}.  Similarly, in searching for dark matter
signatures from the Galactic center or galaxy clusters one must
understand and measure the more standard astrophysical processes that
may lead to signatures that are similar in nature to those expected
from dark matter annihilation.

\underline{\em Extragalactic background light.} In addition to
advancing our understanding of particle acceleration and astrophysical
backgrounds for dark matter searches, the intense gamma-ray beams
generated by AGN and gamma-ray bursts can be used to probe the
intervening space and search for physics beyond the standard
model. Some areas that can be studied include: measuring the
extragalactic background light (EBL), using the EBL to measure the
intergalactic magnetic fields, and searching for axion-like particles
(ALPs) (note, ALPs are not the QCD axion).  The EBL pervades the
universe and is the sum of all the light generated by stars and the
re-radiation of this light in the infrared band by dust \cite{Stecker:2012ta,dominguez2011,dwek2013}
and is therefore sensitive to the star formation history of the universe.
The production of electron-positron pairs from photon-photon
scattering of the EBL with high-energy gamma rays leads to an energy
dependent attenuation length for high-energy gamma rays \cite{Gould:1967zza}.  At the same
time, cosmic rays (if they are accelerated by AGN) will interact with
EBL and CMB along the line of sight and generate secondary gamma rays
at relatively close distances of the observer \cite{Aharonian:1993vz}.  This absorption, with
the inclusion of secondary gamma rays, can be used to measure or
constrain the EBL \cite{dominguez2011,dwek2013}.  Lower limits on the EBL can be established from
galaxy counts \cite{Stecker:2012ta}.  A signature of new physics would be an inconsistency
between these lower limits and the measurements of the TeV spectra
from AGN.  Such a discrepancy could be explained either by the
secondary production of gamma rays from cosmic rays produced at AGN or
by photon-alp mixing mediated by the intergalactic magnetic fields.

\underline{\em Intergalactic magnetic fields.} The origin of the
Galactic magnetic fields remains a mystery.  While astrophysical
dynamos can efficiently amplify pre-existing magnetic fields, the
generation of a magnetic field is difficult \cite{Kandus:2010nw}. The strength of the
magnetic fields in the voids between galaxy clusters should be similar
to the primordial magnetic field. Measurement of AGN spectra and time
delays in the GeV-TeV region have been used to set both lower and
upper bounds on the strength of the IGMF \cite{Plaga:1994hq,Ando:2010rb}.  Current bounds are model
dependent and span a large range of values for the magnetic field \cite{Essey:2011wv}.
Improved measurements of the EBL, the measurement of variability from
distant AGN, and improved determinations of the energy spectra (and
understanding of the intrinsic AGN spectra) are needed to
significantly improve these limits.

\underline{\em Tests of Lorentz invariance violation.}  Experimentally
probing Planck-scale physics, where quantum gravitational effects
become large, is challenging.  A unique signature of such affects
would be the violation of Lorentz invariance (a natural though not
necessary property of theories of quantum gravity) \cite{saslow1998,rovelli2008,solodukhin2011}.  
Short, intense pulses of gamma rays from distant objects such as gamma ray bursts and
active galaxies, provide a laboratory to search for small, energy
dependent, differences in the speed of light.  Current limits have
reached the Planck scale if the energy dependence of the violation is
linear \cite{abdo2009} and $6.4\times10^{10}$ GeV if the violation is quadratic \cite{abromowski2011} 
with energy.  Future instruments could improve upon these limits by at
least a factor of 10 and 50 (respectively) and significantly increase
the sample size used to search for these affects.

\underline{\em TeV Gamma-Ray Instruments.} Ground-based TeV
instruments fall into two classes: extensive air shower (EAS) arrays,
capable of simultaneously viewing the entire overhead sky, and imaging
atmospheric Cherenkov telescopes (IACTs), pointed instruments with
high sensitivity and resolution.  Current IACTs are VERITAS, MAGIC,
and HESS, while the HAWC (under construction) and Tibet arrays are the
only operating EAS arrays.  The next generation of IACT, known as CTA,
will consist of a large array of IACTs with roughly an order of
magnitude greater sensitivity than current instruments.  It is
expected to discover over 1000 sources in the TeV band \cite{cta2011, cta2013}.  The
U.S. portion of the collaboration is proposing to construct $>\sim$26
mid-sized telescopes with a novel optical design that will improve the
sensitivity of CTA by a factor of 2-3 and the resolution by roughly 40\%.

\subsection{Baryogenesis}

According to standard cosmology, the current preponderance of matter
arises during the very early universe from an asymmetry of about one
part per hundred million between the densities of quarks and
antiquarks. This asymmetry must have been created after inflation due
to some physical process known as baryogenesis.  Baryogenesis requires
extending the standard model of particle physics, via some new physics
which must couple to standard model particles and which must be
important during or after the end of inflation. Constraints on the
inflation scale and on the reheat temperature at the end of inflation
give an upper bound on the relevant energy scale for baryogenesis. The
new physics must violate CP (symmetry between matter and antimatter)
as the CP violation in the standard model is insufficient \cite{Gavela:1994dt}. There are a
very large number of theoretical baryogenesis proposals. Some
well-motivated possibilities are:

\underline{\em Leptogenesis} Theoretically, baryon number violation at
high temperatures is rapid in the standard model via nonperturbative
electroweak processes known as sphalerons. Sphalerons conserve the
difference between baryon and lepton numbers, leading to the idea of
leptogenesis \cite{Fukugita:1986hr}. The decay of very heavy neutrinos in the early universe
could occur in a CP violating way, creating a lepton asymmetry that
the sphalerons convert into a baryon asymmetry. Whether and how
leptogenesis could occur can be clarified by intensity frontier
experiments (CP violation and lepton number violation in neutrino
physics) \cite{DiBari:2012fz}, cosmic frontier experiments (most leptogenesis proposals
require a high inflation scale which can be constrained in cosmic
microwave background measurements), and energy frontier experiments \cite{Pilaftsis:2003gt}
(because whether or not other new physics exists has important
implications for leptogenesis).

\underline{\em Affleck-Dine baryogenesis} In supersymmetric theories
condensates of the scalar partners of quarks and leptons have
relatively low energy density and are likely to be present at the end
of inflation \cite{Affleck:1984fy}. The subsequent evolution and decay of the condensates
can produce the baryon asymmetry, and in some models, the dark
matter \cite{Kusenko:1997si,Kusenko:1997vp}. The dark matter could be macroscopic lumps of scalar quarks or
leptons known as Q-balls, which have unusual detection signatures in
cosmic frontier experiments \cite{Kusenko:2005du}. A critical test of this theory is the
search for supersymmetry, primarily via collider experiments.
Instruments such as HAWC and IceCube will be sensitive to extremely
low fluxes of Q-balls - over two orders of magnitude lower than
current limits.  While the non-observation of Q-balls can not rule out
the Affleck-Dine mechanism, the observation of a Q-ball would have a
profound impact on our understanding of the universe.

\underline{\em Electroweak baryogenesis} New non-standard model
particles that are coupled to the Higgs boson can provide a first
order phase transition for electroweak symmetry breaking, which
proceeds via nucleation and expansion of bubbles of broken phase. CP
violating interactions of particles with the expanding bubble walls
can lead to a CP violating particle density in the symmetric phase,
which can be converted by sphalerons into the baryon asymmetry \cite{Cohen:1992zx,Turok:1990zg}. The
baryons then enter the bubbles of broken phase where the sphaleron
rate is negligible. This scenario can be definitively tested via the
search for new particles in high-energy colliders, and via
nonvanishing electric dipole moments for the neutron and for
atoms. Non-standard CP violation in $D$ and $B$ physics may appear in
some models. A non standard Higgs self-coupling is a generic
consequence. The first order phase transition in the early universe
can show up via relic gravitational waves.

Other experiments that can shed light on baryogenesis include searches
for baryon number violation. Neutron anti-neutron oscillations violate
the difference between baryon and lepton numbers, and most
leptogenesis scenarios will not work if such processes are too
rapid. Proton decay would provide evidence for Grand Unification,
which would imply the existence of heavy particles whose decay could
be responsible for baryogenesis, and which is a feature of some
leptogenesis and supersymmetric models.

\subsection{Fundamental nature of spacetime}

Quantum effects of space-time are predicted to originate at the Planck
scale. In standard quantum field theory, their effects are strongly
suppressed at experimentally accessible energies, so space-time is
predicted to behave almost classically, for practical purposes, in
particle experiments. However, new quantum effects of geometry
originating at the Planck scale from geometrical degrees of freedom
not included in standard field theory may have effects on macroscopic
scales \cite{Jacobson:1995ab,Verlinde:2010hp} that could be measured by laser interferometers such as the
holometer \cite{Hogan:2012ib}. In addition, cosmic particles of high energies can probe
departures from Lorenz invariance \cite{amelino1998} and the existence of
extra-dimensions on scales above the LHC.


%%
%% Populate the .bib file with entries from SPIRES Bibtex (preferred)
%% or ADS Bibtex (if no SPIRES entry).
%%  SPIRES will also supply the CITATION line information; please include it.
%%

%\end{document}


==> CF6/executive-summary-v4shorter.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{center}\begin{boldmath}

%\input authorlistCF.tex
%Conveners are also listed separately in authorlist.tex

%\end{boldmath}\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newpage

\section{Cosmic Particles and Fundamental Physics} 


Over the past decade we have witnessed a revolution in our
understanding of the high-energy universe.  Some of the key
discoveries have been:
\begin{itemize}
\item Supernovae have been shown to be a source of Galactic cosmic
  rays \cite{ackermann2013a}.
\item Very high energy neutrinos that are likely to be astrophysical
  in origin have been observed \cite{Aartsen:2013bka}.
\item The GZK suppression in the cosmic-ray flux above $10^{19.5}$ eV
  has been observed \cite{Abbasi:2007sv,Abraham:2008ru}.
\item The positron fraction of the cosmic rays has been measured up to
  300 GeV and provides solid evidence for a high-energy primary source
  of positrons in the Galaxy, either from dark matter annihilation or
  astrophysical processes \cite{adriani2009,,Aguilar:2013qda}.
\item Many sites of astrophysical particle acceleration have been
  directly observed, from supermassive black holes and merging neutron
  stars, to rapidly spinning neutron stars and supernova remnants in
  our Galaxy \cite{Aharonian:2008zza}.
\end{itemize}

These discoveries have been driven by the current generation of
experiments: the IceCube neutrino detector at the South Pole, the
Fermi gamma-ray observatory and the PAMELA  and AMS experiments 
orbiting the earth, the High Resolution FlyÕs Eye and Pierre Auger 
ultra-high-energy cosmic ray experiments, and the H.E.S.S., VERITAS,
MAGIC and Milagro experiments in very high energy gamma rays.  Looking
forward, a new generation of instruments with greater sensitivity and
higher resolution hold the promise of making large advances in our
understanding of astrophysical processes and the fundamental physics
studied with astrophysical accelerators.  The goals for the coming
decade are:
\begin{itemize}
\item Determine the origin of the highest energy particles in the
  universe and understand the acceleration processes at work
  throughout the Universe.
\item Measure particle cross sections at energies unattainable in
  Earth-bound accelerators.
\item Measure the highest energy neutrinos that arise from
  interactions of the ultra-high-energy cosmic rays with the microwave
  background radiation.
\item Measure the extragalactic background light between 1 and 100
  microns to understand the star formation history of the Universe.
\item Measure the mass hierarchy of the neutrinos.
\item Search for physics beyond the standard model encoded in cosmic
  messengers as they cross the Universe.
\item Understand the origins of the matter antimatter asymmetry of the
  Universe.
\item Probe the fundamental nature of spacetime.
\end{itemize}

In many of these areas future progress will depend upon either the
detailed understanding of particle acceleration in the universe or the
development of methods for controlling systematic errors introduced by
our lack of understanding of these processes.  High-resolution gamma
ray measurements (spectral, angular, and temporal) of many objects and
classes of objects are needed to find the source invariant physics
that is the signal for physics beyond the standard model.  Such
measurements in conjunction with measurements at other wavelengths and
with measurements of cosmic rays, neutrinos, and gravity waves will
enable us to understand NatureÕs particle accelerators.

\underline{\bf Recommendations:}
\begin{itemize}
\item Significant U.S. participation in the CTA project \cite{cta2011}.
  U.S. scientists developed the imaging atmospheric Cherenkov
  technique.  Continued leadership in this area is possible with the
  development of novel telescope designs.  A U.S. proposal to more than double
  the number of mid-scale telescopes would result in a sensitivity gain of
  2-3 significantly improving the prospects for the
  indirect detection of dark matter, understanding particle
  acceleration processes, and searching for other signatures of
  physics beyond the standard model.
\item Simultaneous operation of Fermi, HAWC, and VERITAS.
  Understanding particle acceleration and separating astrophysical
  processes from physics beyond the standard model requires
  observations over a broad energy range.  The above three instruments
  will provide simultaneous coverage from 30 MeV to 100 TeV.  HAWC and
  VERITAS will simultaneously view the same sky enabling prompt follow
  up observations of transient phenomena.
\item Construction of the PINGU neutrino detector \cite{aartsen2013} at the South Pole.
  U.S. scientists have been leaders in the field of high-energy
  neutrino observations.  PINGU, by densely instrumenting a portion of
  the IceCube Deep Core array, will lower the energy threshold for
  neutrinos to a few GeV.  This will allow for a measurement of the
  neutrino mass hierarchy using atmospheric neutrinos.
\item Continued operation of the Auger and TA air shower arrays with
  upgrades to enhance the determination of the composition and
  interactions of cosmic rays near the energy of the GZK suppression,
  and flight of the JEM-EUSO mission \cite{TheJEM-EUSO:2013vea} to extend observations of the
  cosmic ray spectrum and anisotropy well beyond the GZK region.
\item Construction of a next-generation ultra-high energy GZK neutrino
  detector either to detect GZK neutrinos \cite{berezinsky2006} and constrain the
  neutrino-nucleon cross section at these energies \cite{Klein2013}, or rule out all
  but the most unfavorable parts of the allowed parameter space.
\end{itemize}

\subsection{Ultra-High-Energy Cosmic Rays}

HiRes  \cite{Abbasi:2007sv}, Auger  \cite{Abraham:2010mj}, and the Telescope Array (TA) \cite{AbuZayyad:2012ru} have established the
existence of a suppression of the spectrum at the highest energies
(above $\sim6\times 10^{19}$ eV ) as predicted by Greisen, Zatsepin,
and Kuzmin (GZK) in 1966 \cite{Greisen:1966jv,Zatsepin:1966jv}.  The GZK suppression is an example of the
profound links between different regimes of physics, connecting the
behavior of the highest-energy particles in the Universe to the cosmic
microwave background radiation, and can be explained by the sub-GeV
scale physics of photo-pion production occurring in the extremely
boosted relativistic frame of the cosmic ray.  A similar phenomenon
occurs for primary nuclei due to excitation of the giant dipole
resonance, resulting in photo-disintegration.  For iron nuclei, this
occurs at about the same energy per particle as the photo-pion process
does for protons.

The composition of cosmic rays and their interactions with air nuclei
may be probed by studies of the depth of shower maximum, $X_{max}$ \cite{ellsworth1982}.
The mean value of $X_{max}$ rises linearly as a function of the log of
the energy, and depends on the nature of the primary particle, the
depth of its first interaction, and the multiplicity and inelasticity
of the interactions as the shower evolves.  Lower energy observations
of $X_{max}$ indicate that the composition becomes lighter as the
energy increases toward $\sim10^{18.3}$ eV \cite{FlysEye93}, which suggests that
extragalactic cosmic rays are mainly protons.  However, at higher
energies the Auger ObservatoryÕs high quality, high-statistics sample
exhibits the opposite trend, along with a decreasing spread in
$X_{max}$ with increasing energy \cite{Abraham:2010mj,Abreu:2013env}.  Using current simulations and
hadronic models tuned with LHC forward data, this implies the
composition is becoming gradually heavier above $10^{18.5}$ eV.  A
trend toward heavier composition could reflect the apparent GZK
suppression being in fact the endpoint of cosmic acceleration in which
there is a maximum magnetic rigidity for acceleration, resulting in
heavy nuclei having the highest energy per particle.

Cosmic rays can be used to probe particle physics at energies far
exceeding those available at the LHC.  An alternative explanation for
the observed behavior of $X_{max}$ is a change in particle
interactions not captured in event generators tuned to LHC data.
Auger measurements using three independent methods find that these
models do not describe observed showers well.  For example, the
observed muon content of showers measured in hybrid events at Auger is
a factor 1.3 to 1.6 higher larger than predicted \cite{AugerMuonICRC13}.  TA also observes a
calorimetric energy that is about 1.3 times higher than that inferred
from their surface detector using these models.  An example of a novel
phenomenon that may explain these observations is the restoration of
chiral symmetry in QCD  \cite{Farrar:2013sfa}.

A critical step in fully understanding the $X_{max}$ observations is
to identify and correct the deficiencies in the beyond-LHC physics
used in modeling showers.  This requires continued operation of
current hybrid detectors such as Auger and TA with upgrades to enable
improved multiparameter studies of composition and interactions on a
shower-by-shower basis.  Enhancements of the surface detectors are
particularly valuable because of the tenfold higher duty cycle than
for fluorescence or hybrid operation.

Observations from space can extend studies of the spectrum and
anisotropy beyond the GZK region with high statistics.  Current
ground-based observatories have observed hints of correlation of
cosmic ray arrival directions with the local distribution of matter \cite{AugerICRC-HL12,TinyakovTAanisoICRC13}, but higher statistics trans-GZK observations are required to identify
sources. In addition, the question of whether the spectrum flattens
again above the GZK suppression or continues to fall will distinguish
between the GZK and acceleration limit scenarios.  The JEM-EUSO
mission has an instantaneous collecting area of $\sim$40  \cite{TheJEM-EUSO:2013vea} times that of
existing ground-based detectors and, taking duty cycle into account,
will increase the collecting area above the GZK suppression energy by
nearly an order of magnitude.

\subsection{Neutrinos}

IceCube has recently reported the detection
of two neutrinos with energies above 1 PeV and 26 events above 30 TeV
with characteristics that point to an astrophysical origin \cite{Aartsen:2013bka}.  These
exciting results herald the beginning of the era of high-energy
neutrino astronomy, and initiating the study of ultra-long baseline
high-energy neutrino oscillations.  Neutrino data complements
observations of cosmic rays and gamma rays due to their origin in the
decays following high-energy hadronic interactions and their weak
couplings.  Several acute issues in particle physics and astrophysics
can be addressed by neutrino experiments.

\underline{\em GZK Neutrinos} Neutrinos are produced by the weak
decays of the mesons and neutrons produced in the interaction of UHE
cosmic rays with the CMB \cite{berezinsky2006}.  The production of these neutrinos takes
place via well-known physics at high Lorentz boost, so robust
predictions of the neutrino flux can be made.  This flux depends on
the composition of the primary cosmic rays and the evolution of the
cosmic ray source density with redshift.  Unlike many searches, there
is a lower limit on the expected flux.  Current detectors such as
IceCube, Auger, RICE, and ANITA
have begun to probe the highest predicted values of the neutrino flux.  Next generation experiments
such as ARA, ARIANNA, and EVA can increase our sensitivity by about
two orders of magnitude, and will either detect GZK neutrinos or rule
out much of the parameter space.  If GZK neutrinos are detected, the
event rate as a function of zenith angle can be used to measure the
neutrino-nucleon cross section and constrain models with enhanced
neutrino interactions at high energy.

\underline{\em Atmospheric Neutrinos and the Neutrino Mass Hierarchy}
PINGU \cite{aartsen2013} is a proposed high-density infill of the IceCube detector with a
reduced energy threshold of a few GeV, employing the rest of IceCube
as an active veto.  PINGU has sensitivity to atmospheric $\nu_{\mu}$
over a range of values of L/E spanned by the variation in the distance
to the production region as a function of zenith angle and the energy
spectrum of atmospheric neutrinos.  Preliminary studies of PINGU
indicate that over these values of L/E, atmospheric $\nu_{\mu}$
oscillations can be used to determine the neutrino mass hierarchy with
3-5$\sigma$ significance with two years of data with a 40 string
detector \cite{aartsen2013} .

\underline{\em Supernova Neutrinos} The Long Baseline Neutrino
Experiment \cite{Adams:2013qkq} will consist of a large (10-35 kTon) liquid argon time
projection chamber located at 4850 feet depth at the Homestake mine in
South Dakota. Collective oscillations of neutrinos as they traverse
the neutrinosphere lead to a spectral swap that leaves a signature in
the energy spectrum of electron neutrinos that is dependent upon the
neutrino mass hierarchy \cite{duan2006}.  In the event of a Galactic supernova,
sufficient numbers of events would be detected to both measure the
neutrino mass hierarchy and to elucidate the supernova mechanism.


\subsection{Gamma Rays}

High-energy gamma rays provide a unique view into the most extreme
environments in the universe, allowing one to probe particle
acceleration processes and the origin of the Galactic and
extragalactic cosmic rays.  Active galactic nuclei (AGN), supermassive
black holes emitting jets of highly relativistic particles along their
rotation axis, have been shown to be sites of particle acceleration \cite{Aharonian:2008zza}.
Outstanding issues in the acceleration processes include: the nature
of the accelerated particles (hadronic or leptonic), the role of shock
acceleration versus magnetic reconnection, and the formation and
collimation of astrophysical jets \cite{boettcher2007}.  Answers to these questions will
come from higher resolution measurements in the GeV-TeV regime,
multi-wavelength campaigns with radio, x-ray, and gamma-ray
instruments, multi-messenger observations with gamma rays, ultra-high
energy cosmic rays, neutrinos, and potentially gravitational
waves. Understanding these extreme environments and how they
accelerate particles is of fundamental interest.  In addition, these
high-energy particle beams, visible from cosmologically interesting
distances, allow us to probe fundamental physics at scales and in ways
that are not possible in earth-bound particle accelerators.

Recently, Fermi \cite{ackermann2013a} and AGILE \cite{Giuliani:2011nx} measured the energy spectra of the supernova
remnants W44 and IC44 Ð the decrease in the gamma-ray flux below the
pion mass in these sources is clear evidence for hadronic
acceleration.  This is the clearest evidence to date that some
Galactic cosmic rays are accelerated in supernova remnants.  The
detection of high-energy neutrinos from a cosmic accelerating would be
a smoking gun signature of hadronic acceleration.  In the absence of
multi-messenger signals multi-wavelength energy spectra (x-ray to TeV)
can test both leptonic models, where the high-energy emission is
derived from inverse Compton scattering of the x-ray synchrotron
emission, and hadronic models, where gamma rays result from pion
decays or proton synchrotron radiation.

\underline{\em Backgrounds to dark matter searches.} Understanding the
origin of the Galactic VHE gamma rays is critical in the
interpretation of some signatures of dark matter annihilation.  The
recent results from PAMELA \cite{adriani2009} and AMS \cite{Aguilar:2013qda} of the increasing positron fraction
with energy is a clear signal that the current model of secondary
production and transport through the Galaxy is not correct.  There are
three potential explanations for this signal: a new astrophysical
source of positrons \cite{Hooper:2008kg}, modified propagation of cosmic rays or secondary
production in the source \cite{Zirakashvili:2011sc}, or dark matter annihilation \cite{turner1990}.  An
astrophysical source of positrons, pulsar wind nebula (PWN), is now
known to also lead to an increasing positron fraction at high
energies.  Observations of the Geminga PWN in the TeV band by Milagro \cite{abdo2009b}
have been used to normalize the flux of positrons in our local
neighborhood from this source.  The calculated positron fraction is an
excellent match to the data \cite{yuksel2009}.  Similarly, in searching for dark matter
signatures from the Galactic center or galaxy clusters one must
understand and measure the more standard astrophysical processes that
may lead to signatures that are similar in nature to those expected
from dark matter annihilation.

\underline{\em Extragalactic background light.} In addition to
advancing our understanding of particle acceleration and astrophysical
backgrounds for dark matter searches, the intense gamma-ray beams
generated by AGN and gamma-ray bursts can be used to probe the
intervening space and search for physics beyond the standard
model. Some areas that can be studied include: measuring the
extragalactic background light (EBL), using the EBL to measure the
intergalactic magnetic fields, and searching for axion-like particles
(ALPs) (note, ALPs are not the QCD axion).  The EBL pervades the
universe and is the sum of all the light generated by stars and the
re-radiation of this light in the infrared band by dust \cite{dominguez2011}
and is therefore sensitive to the star formation history of the universe.
The production of electron-positron pairs from photon-photon
scattering of the EBL with high-energy gamma rays leads to an energy
dependent attenuation length for high-energy gamma rays \cite{Gould:1967zza}.  At the same
time, cosmic rays (if they are accelerated by AGN) will interact with
EBL and CMB along the line of sight and generate secondary gamma rays
at relatively close distances of the observer \cite{Aharonian:1993vz}.  This absorption, with
the inclusion of secondary gamma rays, can be used to measure or
constrain the EBL \cite{dominguez2011}.  Lower limits on the EBL can be established from
galaxy counts.  A signature of new physics would be an inconsistency
between these lower limits and the measurements of the TeV spectra
from AGN.  Such a discrepancy could be explained either by the
secondary production of gamma rays from cosmic rays produced at AGN or
by photon-alp mixing mediated by the intergalactic magnetic fields.

\underline{\em Intergalactic magnetic fields.} The origin of the
Galactic magnetic fields remains a mystery.  While astrophysical
dynamos can efficiently amplify pre-existing magnetic fields, the
generation of a magnetic field is difficult \cite{Kandus:2010nw}. The strength of the
magnetic fields in the voids between galaxy clusters should be similar
to the primordial magnetic field. Measurement of AGN spectra and time
delays in the GeV-TeV region have been used to set both lower and
upper bounds on the strength of the IGMF \cite{Plaga:1994hq}.  Current bounds are model
dependent and span a large range of values for the magnetic field.
Improved measurements of the EBL, the measurement of variability from
distant AGN, and improved determinations of the energy spectra (and
understanding of the intrinsic AGN spectra) are needed to
significantly improve these limits.

\underline{\em Tests of Lorentz invariance violation.}  Experimentally
probing Planck-scale physics, where quantum gravitational effects
become large, is challenging.  A unique signature of such affects
would be the violation of Lorentz invariance (a natural though not
necessary property of theories of quantum gravity) \cite{solodukhin2011}.  
Short, intense pulses of gamma rays from distant objects such as gamma ray bursts and
active galaxies, provide a laboratory to search for small, energy
dependent, differences in the speed of light.  Current limits have
reached the Planck scale if the energy dependence of the violation is
linear \cite{abdo2009} and $6.4\times10^{10}$ GeV if the violation is quadratic \cite{abromowski2011} 
with energy.  Future instruments could improve upon these limits by at
least a factor of 10 and 50 (respectively) and significantly increase
the sample size used to search for these affects.

\underline{\em TeV Gamma-Ray Instruments.} Ground-based TeV
instruments fall into two classes: extensive air shower (EAS) arrays,
capable of simultaneously viewing the entire overhead sky, and imaging
atmospheric Cherenkov telescopes (IACTs), pointed instruments with
high sensitivity and resolution.  Current IACTs are VERITAS, MAGIC,
and HESS, while the HAWC (under construction) and Tibet arrays are the
only operating EAS arrays.  The next generation of IACT, known as CTA,
will consist of a large array of IACTs with roughly an order of
magnitude greater sensitivity than current instruments.  It is
expected to discover over 1000 sources in the TeV band \cite{cta2013}.  The
U.S. portion of the collaboration is proposing to more than double the number of mid-sized telescopes 
to over 50 using a novel optical design that will improve the
sensitivity of CTA by a factor of 2-3 (a result of improved angular resolution of the new telescopes 
and an increase in the number of telescopes).

\subsection{Baryogenesis}

According to standard cosmology, the current preponderance of matter
arises during the very early universe from an asymmetry of about one
part per hundred million between the densities of quarks and
antiquarks. This asymmetry must have been created after inflation due
to some physical process known as baryogenesis.  Baryogenesis requires
extending the standard model of particle physics, via some new physics
which must couple to standard model particles and which must be
important during or after the end of inflation. Constraints on the
inflation scale and on the reheat temperature at the end of inflation
give an upper bound on the relevant energy scale for baryogenesis. The
new physics must violate CP (symmetry between matter and antimatter)
as the CP violation in the standard model is insufficient \cite{Gavela:1994dt}. There are a
very large number of theoretical baryogenesis proposals. Some
well-motivated possibilities are:

\underline{\em Leptogenesis} Theoretically, baryon number violation at
high temperatures is rapid in the standard model via nonperturbative
electroweak processes known as sphalerons. Sphalerons conserve the
difference between baryon and lepton numbers, leading to the idea of
leptogenesis \cite{Fukugita:1986hr}. The decay of very heavy neutrinos in the early universe
could occur in a CP violating way, creating a lepton asymmetry that
the sphalerons convert into a baryon asymmetry. Whether and how
leptogenesis could occur can be clarified by intensity frontier
experiments (CP violation and lepton number violation in neutrino
physics) \cite{DiBari:2012fz}, cosmic frontier experiments (most leptogenesis proposals
require a high inflation scale which can be constrained in cosmic
microwave background measurements), and energy frontier experiments \cite{Pilaftsis:2003gt}
(because whether or not other new physics exists has important
implications for leptogenesis).

\underline{\em Affleck-Dine baryogenesis} In supersymmetric theories
condensates of the scalar partners of quarks and leptons have
relatively low energy density and are likely to be present at the end
of inflation \cite{Affleck:1984fy}. The subsequent evolution and decay of the condensates
can produce the baryon asymmetry, and in some models, the dark
matter \cite{Kusenko:1997si,Kusenko:1997vp}. The dark matter could be macroscopic lumps of scalar quarks or
leptons known as Q-balls, which have unusual detection signatures in
cosmic frontier experiments \cite{Kusenko:2005du}. A critical test of this theory is the
search for supersymmetry, primarily via collider experiments.
Instruments such as HAWC and IceCube will be sensitive to extremely
low fluxes of Q-balls - over two orders of magnitude lower than
current limits.  While the non-observation of Q-balls can not rule out
the Affleck-Dine mechanism, the observation of a Q-ball would have a
profound impact on our understanding of the universe.

\underline{\em Electroweak baryogenesis} New non-standard model
particles that are coupled to the Higgs boson can provide a first
order phase transition for electroweak symmetry breaking, which
proceeds via nucleation and expansion of bubbles of broken phase. CP
violating interactions of particles with the expanding bubble walls
can lead to a CP violating particle density in the symmetric phase,
which can be converted by sphalerons into the baryon asymmetry \cite{Cohen:1992zx}. The
baryons then enter the bubbles of broken phase where the sphaleron
rate is negligible. This scenario can be definitively tested via the
search for new particles in high-energy colliders, and via
nonvanishing electric dipole moments for the neutron and for
atoms. Non-standard CP violation in $D$ and $B$ physics may appear in
some models. A non standard Higgs self-coupling is a generic
consequence. The first order phase transition in the early universe
can show up via relic gravitational waves.

Other experiments that can shed light on baryogenesis include searches
for baryon number violation. Neutron anti-neutron oscillations violate
the difference between baryon and lepton numbers, and most
leptogenesis scenarios will not work if such processes are too
rapid. Proton decay would provide evidence for Grand Unification,
which would imply the existence of heavy particles whose decay could
be responsible for baryogenesis, and which is a feature of some
leptogenesis and supersymmetric models.

\subsection{Fundamental nature of spacetime}

Quantum effects of space-time are predicted to originate at the Planck
scale. In standard quantum field theory, their effects are strongly
suppressed at experimentally accessible energies, so space-time is
predicted to behave almost classically, for practical purposes, in
particle experiments. However, new quantum effects of geometry
originating at the Planck scale from geometrical degrees of freedom
not included in standard field theory may have effects on macroscopic
scales \cite{Verlinde:2010hp} that could be measured by laser interferometers such as the
holometer \cite{Hogan:2012ib}. In addition, cosmic particles of high energies can probe
departures from Lorenz invariance and the existence of
extra-dimensions on scales above the LHC.


%%
%% Populate the .bib file with entries from SPIRES Bibtex (preferred)
%% or ADS Bibtex (if no SPIRES entry).
%%  SPIRES will also supply the CITATION line information; please include it.
%%

%\end{document}


==> CF6/introduction.tex <==
\section{Overview}

The Cosmic Frontier number 6, named Cosmic Probes of Fundamental
Physics, was charged with summarizing current knowledge and
identifying future opportunities (both experimental and theoretical)
in the use of astrophysical probes of fundamental physics. Because of
the breadth of this area of research CF6 has been subdivided into 3
main topical areas: 

\begin{itemize}
\item	CF6-A Cosmic Rays, Gamma Rays and Neutrinos (conveners: Gus Sinnis, Tom Weiler)
\item	CF6-B The Matter of the Cosmological Asymmetry (convener: Ann Nelson)
\item	CF6-C Exploring the Basic Nature of Space and Time (conveners: Aaron Chou, Craig Hogan)
\end{itemize}

We received [[XX]] whitepapers addressing the current challenges and
future opportunities in each of these fields as they relate to the
other frontiers of high energy physics.


\subsection{Physics Motivation}

The Universe has a large number of cosmic accelerators that can give
insight into particle interactions and fundamental
physics. Understanding the flux and energy reach of particles that
reach Earth from remote places in the cosmos give an opportunity to
probe physics beyond the reach of artificial laboratories. In addition
to probing the limits of known interactions with cosmic probes, high
sensitivity experiments can find rare long lived new particles that
can change current views on the basic components of matter.

The basic question of the matter-antimatter is another focus of this
cosmic frontier. [[Ann may want to add some sentences here]]

Quantum effects of space-time are predicted to originate at the Planck
scale. In standard quantum eld theory, their effects are strongly
suppressed at experimentally accessible energies, so space-time is
predicted to behave almost classically, for practical purposes, in
particle experiments. However, new quantum effects of geometry
originating at the Planck scale| from geometrical degrees of freedom
not included in standard field theory| may have effects on macroscopic
scales that could be measured by laser interferometers, such as the
bolometer. In addition, cosmic particles of high energies can probe
departures from Lorenz invariance and the existence of
extra-dimensions on scales above the LHC.


 

\subsection{Summary of topical areas addressed }

\subsubsection{CF6-A Cosmic Rays, Gamma Rays and
  Neutrinos}

Cosmic rays, gamma rays, and neutrinos from
astrophysical sources can be used to probe fundamental symmetries,
particle interactions at energies not attainable on Earth, and
understand the nature of particle acceleration in the cosmos. CF6-A
encompasses the following topical areas:
 The Physics of Interactions
Beyond Laboratory Energies (hadronic and weak interactions at high
energies)
 Cosmic Particle Acceleration (origin of the cosmic
radiation from GeV to ZeV, astrophysical backgrounds to fundamental
physics)
 Cosmic Standard Model (SM) Particles as Probes of
Fundamental Physics (violation of Lorentz invariance, extra
dimensions, axions)
 New Particles (anti-nuclei, strangelets,
Q-Balls, primordial black holes)
 Neutrino Physics from Astrophysics
(in conjunction with the Intensity Frontier IF3: neutrino mass
hierarchy, leptonic CP violation, neutrino interactions in supernovae,
non-standard neutrino interactions with matter)

The relevant
experiments for CF6-A are listed in TABLE 1. This field is ripe for
new discoveries. Recent examples include the detection by the Fermi
and AGILE space missions of a pion-zero decay produced gamma-ray
signal in supernova remnants W44 and IC44 \cite{FermiW44}; the first
detection of 10 TeV to PeV neutrinos by Icecube \cite{BertErnie}; and
the precise positron fraction measurement of the Alpha Magnetic
Spectrometer \cite{AMSpositrons}. The 


\subsubsection{CF6-B The
  Matter of the Cosmological Asymmetry}

The cosmological asymmetry
between baryons and anti-baryons is one of the strongest pieces of
evidence for physics beyond the standard model. There are diverse
theoretical proposals for new physics at a range of energy scales,
most of which include new sources of CP violation, and either
additional baryon or lepton number violation. There are plausible
theories with implications for experiments at all three
frontiers. Leptogenesis theories predict new CP violation in the
neutrino sector. Grand Unified theories predict proton
decay. Electroweak baryogenesis models predict a cosmological phase
transition which leaves traces in gravitational wave and CMB
experiments, and new collider physics at or below a TeV.

Survey
what we may expect to learn about the origin of matter from searches
at ongoing, planned and proposed facilities such as the LHC, ILC,
CLIC, muon collider, B-factories, neutrino experiments, gravitational
wave experiments and CMB experiments.

\subsubsection{CF6-C
  Exploring the Basic Nature of Space and Time}

Space and time may
be quantized at the Planck scale. Effects from this extremely
high-energy realm may be studied through gravitational waves from the
early universe and holographic noise.

Survey what we may expect to
learn about the GUT and Planck energy scale with gravitational waves
and holographic noise. Survey the theory and ongoing, planned, and
proposed gravitational wave and holographic noise
experiments. Examples of relevant experiments include the Holometer,
LIGO, LISA, and CMB probes of early universe gravitational wave
(covered in Dark Energy and CMB.)

\subsection{Upcoming Opportunities (Next Generation Facilities) }

\subsubsection{(short list that addresses questions and physics issues)}

\subsection{Answers to Tough Questions}


==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

